Beyond Model Adaptation at Test Time: A Survey

Machine learning algorithms have achieved remarkable success across various disciplines, use cases and applications, under the prevailing assumption that training and test samples are drawn from the same distribution. Consequently, these algorithms struggle and become brittle even when samples in the test distribution start to deviate from the ones observed during training. Domain adaptation and domain generalization have been studied extensively as approaches to address distribution shifts across test and train domains, but each has its limitations. Test-time adaptation, a recently emerging learning paradigm, combines the benefits of domain adaptation and domain generalization by training models only on source data and adapting them to target data during test-time inference. In this survey, we provide a comprehensive and systematic review on test-time adaptation, covering more than 400 recent papers. We structure our review by categorizing existing methods into five distinct categories based on what component of the method is adjusted for test-time adaptation: the model, the inference, the normalization, the sample, or the prompt, providing detailed analysis of each. We further discuss the various preparation and adaptation settings for methods within these categories, offering deeper insights into the effective deployment for the evaluation of distribution shifts and their real-world application in understanding images, video and 3D, as well as modalities beyond vision. We close the survey with an outlook on emerging research opportunities for test-time adaptation.

==> 5_datasets.tex <==
\section{Evaluations and Datasets}
\label{sec:dataset}

In this section, we talk about the evaluation methods of test-time adaptation and summarize some most commonly-used datasets. We also provide comparisons of some representative methods.

\subsection{Evaluations}
\textbf{Single target distribution.}
As aforementioned, test-time adaptation aims to train the model on only source data and adapt it to unseen target data along with inference. 
Therefore, the evaluation methods of test-time adaptation are quite straightforward.
After obtaining the source-trained model on single or multiple source distributions, adaptation and evaluation are achieved with the source-trained model and the target samples according to the adaptation settings, e.g., batch-wise, sample-wise, or online. 
Sample-wise adaptation makes adjustments and predictions on each single target sample, while batch-wise adaptation operates on each batch of target samples.
Online adaptation incrementally adjusts and makes predictions on the target data as it becomes available. As a result, the performance of online target samples is expected to improve progressively over time.
The performance metric of test-time adaptation depends on the specific task and dataset. For instance, on the most wide-used classification tasks, the evaluation metric is the top-1 accuracy.

\textbf{Changing target distribution.}
To evaluate the test-time adaptation methods in continually changing environments, some other settings are proposed \cite{gong2022note, niu2023towards, song2023ecotta, wang2022continual}.
These methods also evaluate the models on the commonly used datasets but try to mimic a dynamic environment at test time.
One of the settings is the continual test-time adaptation \cite{wang2022continual}, where the model is continually adapted to each corruption type sequentially without resetting the model.
The other settings include temporally correlation \cite{gong2022note}, imbalanced label shifts \cite{niu2023towards}, mixture of multiple target distributions \cite{niu2022efficient}, and single-sample adaptation \cite{gao2022back, khurana2021sita, niu2023towards, xiao2022learning}.

\subsection{Datasets}
\label{sec:datasets}

The main research on test-time adaptation is on the image classification task. Here we summarize the common classification datasets and provide comparisons of some representative test-time adaptation methods on the most widely-used ones.
The datasets for other applications are provided in Section \ref{application}.
The current test-time adaptation methods train the model on either a single source distribution or multiple source distributions.
We provide the summary and comparisons of both single-source and multi-source datasets.

\subsubsection{Single source distribution}

\textbf{Digits datasets.}
Digit adaptation is widely used in domain adaptation, where different distributions are different datasets, e.g., MNIST \cite{lecun1998gradient}, MNIST-M \cite{ganin2015unsupervised}, SVHN \cite{netzer2011reading}, and USPS \cite{hull1994database}.
The distributions have the same label space with 10 categories.
Following \cite{wang2021tent}, most test-time adaptation methods on digits datasets train the model on SVHN. The source-trained model is then adapted and evaluated on different target distributions, MNIST, MNIST-M, and USPS.

\textbf{Corruption datasets.}
The corruption datasets \cite{hendrycks2019benchmarking}, e.g., CIFAR-10-C, CIFAR-100-C, and ImageNet-C, are widely used in many test-time adaptation methods.
The model is trained on the original dataset, e.g., CIFAR \cite{krizhevsky2009learning} or ImageNet \cite{russakovsky2015imagenet}.  
The target distributions are obtained by applying 15 types of corruption at five severity levels on the original test set of the datasets, as shown in Figure \ref{corruption}.

\begin{figure}[t]
\centering
\vspace{-2mm}
\includegraphics[width=0.9\linewidth]{figures/corruption.png}
% \vspace{-6mm}
\caption{\textbf{Examples of the corruption types in the image corruption datasets.}}
\label{corruption}
% \vspace{-5mm}
\end{figure}


\begin{table}[t]
\begin{center}
\vspace{-2mm}
\caption{\textbf{Top-1 errors on CIFAR-10-C, CIFAR-100-C, and CIFAR-10.1.} Results with \dag~ are from \cite{zhang2021memo}. \ddag~ denotes the result reimplemented by \cite{liu2021ttt++}. 
}
\label{cifar}
% \vspace{-2mm}
	\resizebox{1\columnwidth}{!}{%
		\setlength\tabcolsep{4pt} 
\begin{tabular}{lccc}
\toprule
        Methods & CIFAR-10-C & CIFAR-100-C & CIFAR-10.1 \\ 
        \midrule
        \rowcolor{mColor2}
        \multicolumn{4}{l}{\textbf{ResNet-26}}\\
        Source-trained \dag & 40.8 & 67.2 & 18.4 \\
        Sun et al. \cite{sun2020test} & 17.5 & 45.0 & 15.9 \dag \\
        Wang et al. \cite{wang2021tent} & 14.3 & 37.3 & - \\ 
        Zhang et al. \cite{zhang2021memo} & 19.6 & - & 14.1 \\ 
        Zhou et al. \cite{zhou2021bayesian} & 12.2 & 31.7 & - \\
        Goyal et al. \cite{goyal2022test} & 12.5 & 36.1 & - \\ 
        \rowcolor{mColor2}
        \multicolumn{4}{l}{\textbf{ResNet-50}}\\
        Source-trained \ddag & 29.1 & 61.2 & 12.1 \\
        Sun et al. \cite{sun2020test} \ddag & 14.3 & 40.4 & 11.0 \\
        Wang et al. \cite{wang2021tent} \ddag & 12.6 & 36.3 & 13.4 \\ 
        Jang et al. \cite{jang2022test} & 13.1 & 37.8 & - \\
        Tomar et al. \cite{tomar2023tesla} & 12.1 & 37.3 & - \\ % 53.1 for IN-C
        Su et al. \cite{su2022revisiting} & 10.7 & 34.8 & 9.2 \\ % 50.1 for IN-C
        Liu et al. \cite{liu2021ttt++} & 9.8 & 34.1 & 9.5 \\
\bottomrule
\end{tabular}
}
\end{center}
\end{table}


\begin{table}[t]
\begin{center}
\vspace{-2mm}
\caption{\textbf{Top-1 errors on ImageNet-C, ImageNet-A, and ImageNet-R.} 
}
\label{imagenet}
% \vspace{-2mm}
	\resizebox{1\columnwidth}{!}{%
		\setlength\tabcolsep{4pt} 
\begin{tabular}{lccc}
\toprule
        Methods & ImageNet-C & ImageNet-A & ImageNet-R \\ 
        \midrule
        \rowcolor{mColor2}
        % \multicolumn{4}{l}{\textbf{ResNet-18}}\\
        % Baseline & 40.8 & 67.2 & 59.5 \\
        % Sun et al. \cite{sun2020test} & 17.5 & 45.0 & 44.0 \\
        % Wang et al. \cite{wang2021tent} & 14.3 & 37.3 & 44.0 \\ 
        % Zhang et al. \cite{zhang2021memo} & 19.6 & - & 40.6 \\ 
        \rowcolor{mColor2}
        \multicolumn{4}{l}{\textbf{ResNet-50}}\\
        Source-trained & 80.3 & 63.9 & 100.0 \\
        % Sun et al. \cite{sun2020test} & 44.0 & 45.0 & 44.0 \\
        % Gandelsman et al. \cite{gandelsmantest2022test} & & & \\
        Wang et al. \cite{wang2021tent} & 44.0 & 46.9 & 96.7 \\ 
        Khurana1 et al. \cite{khurana2021sita} & 74.5 & 59.7 & 98.9 \\ % single sample norm
        Zhang et al. \cite{zhang2021memo} & 49.8 & 49.2 & 94.8 \\ 
        Niu et al. \cite{niu2022efficient} & 52.1 & 54.8 & - \\
        Goyal et al. \cite{goyal2022test} & 45.4 & - & - \\
        Zhou et al. \cite{zhou2021bayesian} & 37.0 & - & - \\
        Schneider et al. \cite{schneider2020improving} & 35.5 & 48.9 & - \\ % normalization
        % Gao et al. \cite{gao2022back} & 27.3 & - & - \\ % sample adaptation, image wise adaptation
\bottomrule
\end{tabular}
}
\end{center}
\end{table}

\textbf{Other single-source datasets.}
In addition to the corruption, there are also some other test-time adaptation datasets based on real image benchmarks like CIFAR and ImageNet.
CIFAR-10.1 \cite{recht2018cifar} is a test set for CIFAR-10 that consists of images not present in the original CIFAR-10 dataset.
While both datasets share the same 10 classes, the images in CIFAR-10.1 are selected to be more challenging and less similar to the CIFAR-10 training set.
Thus, there is natural distributional shifts between the two datasets.
ImageNet-A \cite{hendrycks2021natural} also focuses on natural distribution shifts, which contain real-world, unmodified, and naturally occurring examples of ImageNet classes.
ImageNet-R \cite{hendrycks2021many} considers distribution shifts of various renditions of the original images, e.g., paintings, cartoons, etc.

% \textcolor{blue}{Vis-DA?}

\textbf{Comparisons.}
In single-source test-time adaptation methods, the models are trained on the original datasets, CIFAR or ImageNet, and adapted to the shifted distributions, CIFAR-C, CIFAR-10.1, or ImageNet-C, ImageNet-R.
We provide the comparisons of distribution shifts on CIFAR and ImageNet in Table~\ref{cifar} and Table~\ref{imagenet}, respectively.
The model fine-tuning methods \cite{sun2020test, wang2021tent, zhou2021bayesian, goyal2022test, zhang2021memo} and normalization-based methods \cite{schneider2020improving, mirza2022norm, lim2023ttn}, as well as some sample generation methods \cite{gao2022back}, usually conduct experiments on the corruption datasets, e.g., CIFAR-C and ImageNet-C, and achieve good results on these datasets.
The model-inferring-based methods \cite{dubey2021adaptive, iwasawa2021test, xiao2022learning} usually require multiple source distributions during training.
Therefore, most of these methods do not provide results on single-source training.
Xiao et al. \cite{xiao2022learning} provide some single-source results on digit datasets, which are not as good as the model fine-tuning methods \cite{wang2021tent}.

\begin{table}[t]
\begin{center}
\vspace{-2mm}
\caption{\textbf{Top-1 errors of continual test-time adaptation on corruption datasets. Methods with \dag~ are reproduced by \cite{wang2022continual}.} The experiments on CIFAR-10, CIFAR-100, and ImageNet are conducted on WideResNet-28, ResNeXt-29, and ResNet-50, respectively.
The continual test-time adaptation methods perform better than the common method \cite{wang2021tent}.
}
\label{continual}
% \vspace{-2mm}
	\resizebox{1\columnwidth}{!}{%
		\setlength\tabcolsep{4pt} 
\begin{tabular}{lccc}
\toprule
        Methods & CIFAR-10-C & CIFAR-100-C & ImageNet-C \\ 
        \midrule
        % \rowcolor{mColor2}
        % \multicolumn{4}{l}{\textbf{ResNet-50}}\\
        Source-trained \dag & 43.5 & 46.4 & 82.4 \\
        Wang et al. \cite{wang2021tent} \dag & 20.7 & 60.9 & 66.5 \\  %ResNeXt-29
        Wang et al. \cite{wang2022continual} & 16.2 & 32.5 & 63.0 \\
        Brahma et al. \cite{brahma2022probabilistic} & 16.0 & 31.5 & 62.7 \\
        Song et al. \cite{song2023ecotta} & 14.4 & 39.2 & 54.4 \\ %Res50 for cifar and augmix for imagenet. 
        Niu et al. \cite{niu2022efficient} & 19.7 & 40.8 & 58.6 \\
        Hong et al. \cite{hong2023mecta} & 19.3 & 33.8 & 56.7 \\
        Chakrabarty et al. \cite{chakrabarty2023sata} & 16.1 & 30.3 & 60.1 \\
        Hong et al. \cite{hong2023mecta} + Niu et al. \cite{niu2022efficient} & 13.0 & 33.4 & 43.3 \\
\bottomrule
\end{tabular}
}
\end{center}
\end{table}

Table \ref{continual} shows the results of the continual test-time adaptation setting. 
Compared with the common setting in Table \ref{cifar} and Table \ref{imagenet}, the common test-time adaptation methods, e.g., Tent \cite{wang2021tent}, performs worse since the model encounters catastrophic forgetting.
As shown in Table \ref{continual}, The continual test-time adaptation settings perform obviously better than the common methods.
To deal with catastrophic forgetting, these methods require to recover the model parameters. 
Therefore, many recent methods focus on improving the efficiency \cite{hong2023mecta, niu2022efficient, song2023ecotta}.

Moreover, the methods based on single-sample adaptation, e.g., with data augmentation \cite{khurana2021sita, zhang2021memo}, alternative normalization layers \cite{gong2022note, niu2023towards}, and sample generation \cite{gao2022back}, may underperform the other methods in Table \ref{cifar} and \ref{imagenet}. 
But these methods perform well with small amounts of samples, which is important in complex environments with fewer samples or samples from different distributions.
As shown in Table \ref{singlesample}, the typical model adaptation methods Tent \cite{wang2021tent} struggles with small numbers of target samples during adaptation, especially single samples.
The performance on ImageNet-C is even worse than the source-trained model.
By contrast, the single-sample adaptation methods show significant improvements with adaptation on only single target samples.

\begin{table}[t]
\begin{center}
\vspace{-2mm}
\caption{\textbf{Top-1 errors of adaptation with small amounts of samples on ImageNet-C.}
Methods with \dag~ are reproduced by \cite{gao2022back}. The sample adaptation method \cite{gao2022back} and method without BatchNorm layers \cite{niu2023towards} achieve obvious improvement on single sample test-time adaptation.
}
\label{singlesample}
% \vspace{-2mm}
	\resizebox{1\columnwidth}{!}{%
		\setlength\tabcolsep{4pt} 
\begin{tabular}{lcc}
\toprule
        Methods & Number of samples & ImageNet-C \\ 
        \midrule
        % \rowcolor{mColor2}
        % \multicolumn{4}{l}{\textbf{ResNet-50}}\\
        Source-trained & - & 80.3 \\
        Wang et al. \cite{wang2021tent} \dag & 1 & 97.0 \\ 
        Wang et al. \cite{wang2021tent} \dag & 64 &  92.4 \\ 
        Nie et al. \cite{nie2022diffusion} \dag & 1 & 83.2 \\
        Mirza et al. \cite{mirza2022norm} & 1 & 78.2 \\
        Zhang et al. \cite{zhang2021memo} \dag & 1 & 75.3 \\ 
        Khurana1 et al. \cite{khurana2021sita} & 1 & 75.0 \\ % single sample norm
        Gao et al. \cite{gao2022back} & 1  & 70.3 \\ % sample adaptation, image wise adaptation
        Niu et al. \cite{niu2023towards} & 1 & 65.5 \\
\bottomrule
\end{tabular}
}
\end{center}
\end{table}


\subsubsection{Multiple source distributions}
Some test-time adaptation methods train the source model on multiple source domains. 
For instance, the methods learn extra models to extract domain information \cite{dubey2021adaptive, iwasawa2021test} or require to mimic domain shifts during training \cite{du2020metanorm, xiao2022learning}.
In these methods, domain generalization datasets are utilized widely.

\textbf{Domain generalization datasets.}
Domain generalization has been investigated for a quite long time and there were various datasets proposed, e.g., PACS, Office-Home, and DomainNet, most of which have multiple distributions from different domains.
% We conduct our experiments on five widely used datasets for domain generalization, \textbf{PACS} \cite{li2017deeper}, \textbf{Office-Home} \cite{venkateswara2017deep}, \textbf{DomainNet} \cite{peng2019moment}, and \textbf{Rotated MNIST and Fashion-MNIST}.
PACS \cite{li2017deeper} consists of 9,991 images of seven classes from four domains, i.e., \textit{photo}, \textit{art-painting}, \textit{cartoon}, and \textit{sketch}.
\textit{VLCS} \cite{fang2013video} consists of 5 classes from 4 different datasets: Pascal, LabelMe, Caltech, and SUN with 10,729 samples. 
Office-Home \cite{venkateswara2017deep} also contains four domains, i.e., \textit{art}, \textit{clipart}, \textit{product}, and \textit{real-world}, which totally have 15,500 images of 65 categories. 
\textit{TerraIncognita} \cite{beery2018recognition} has 4 domains taken by camera from 4 different locations. The dataset includes 24,778 samples of 10 categories.
DomainNet \cite{peng2019moment} is more challenging since it has six domains i.e., \textit{clipart}, \textit{infograph}, \textit{painting}, \textit{quickdraw}, \textit{real}, \textit{sketch}, with 586,575 examples of 345 classes.
The methods conducted on these domain generalization datasets follow the ``leave-one-out'' protocol \cite{li2017deeper}, where one domain is utilized as the target domain and the rest domains as the source ones.
The source model is trained on all source domains and then adapted and evaluated on the target domain.

% \textcolor{blue}{Wilds?}

\begin{table}[t]
\begin{center}
\vspace{-2mm}
\caption{\textbf{Classification accuracy on domain generalization datasets.}. Recent sample adaptation methods \cite{pandey2021generalization, xiao2023energy} achieve even better performance than model adaptation methods on these multiple source domain datasets.
}
\label{dgdata}
% \vspace{-2mm}
	\resizebox{1\columnwidth}{!}{%
		\setlength\tabcolsep{4pt} 
\begin{tabular}{lccccc}
\toprule
        Methods & VLCS & PACS & Office-Home & DomainNet & TerraIncognita  \\ 
        \midrule
        \rowcolor{mColor2}
        \multicolumn{6}{l}{\textbf{ResNet-18}}\\
        Source-trained \dag & 40.8 & 67.2 & 18.4 \\
        Wang et al. \cite{wang2021tent}\dag & 72.3 & 83.9 & 62.7 & - &  36.9  \\
        Iwasawa et al. \cite{iwasawa2021test} & 74.5 & 81.4 & 63.2 & - & 39.5  \\
        Jang et al. \cite{jang2022test} & 77.3 & 81.9 & 63.7 & - & 42.6  \\
        Chen et al. \cite{chen2023improved} & 76.9 & 83.8 & 62.0 & 34.9 & 43.2 \\
        Xiao et al. \cite{xiao2022learning} & - & 84.2  & 66.0 & - & - \\
        Xiao et al. \cite{xiao2023energy} & - & 85.1 & 66.8 & - & - \\ 
        Pandey et al. \cite{pandey2021generalization} & - & 86.7 & 68.6 & - & - \\ 
        \rowcolor{mColor2}
        \multicolumn{6}{l}{\textbf{ResNet-50}}\\
        Source-trained \ddag & 76.7 & 83.2 & 67.2 & 41.1 & 46.2 \\
        Wang et al. \cite{wang2021tent}\dag & 75.4&  87.0 &  66.9 &  - &  42.6  \\ 
        Dubey et al. \cite{dubey2021adaptive} & 78.0 & 84.1 & 67.9 & 43.6 & 47.3 \\ 
        Iwasawa et al. \cite{iwasawa2021test} & 76.0 & 85.1 & 68.2 & - & 44.6 \\
        Jang et al. \cite{jang2022test} & 77.7 & 84.1 & 68.6 & - & 47.4  \\
        Sun et al. \cite{sun2022dynamic} & - & 86.2 & 72.1 & 46.9 & - \\
        Xiao et al. \cite{xiao2022learning} & 78.6 & 87.5 & 71.1 & - & 48.5 \\
        Xiao et al. \cite{xiao2023energy} & - & 88.1 & 72.3 & 45.0 & -\\ 
\bottomrule
\end{tabular}
}
\end{center}
\end{table}


\textbf{Comparisons.}
For multi-source test-time adaptation, the models are trained on all source distributions and then adapted and evaluated on the target one.
As shown in Table~\ref{dgdata}, most of the model-inferring methods  conduct experiments on domain generalization datasets. 
As aforementioned, some model-inferring methods underperform fine-tuning methods in single-source test-time adaptation.
One reason is that model-inferring methods usually require multiple source distributions to learn the ability to generate specific model parameters for different distributions.
Thus, the model-inferring methods perform better for multi-source test-time adaptation, compared with the fine-tuning-based methods \cite{jang2022test, wang2021tent}.
The generation-based sample adaptation methods \cite{pandey2021generalization, xiao2023energy} also achieve good performance on domain generalization datasets, even better than the model inferring methods on some datasets.


% table of different methods with datasets, evaluations, and adaptation strategies.

% code package.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> others.tex <==
% \begin{table*}[t]
% \begin{center}
% \vspace{-2mm}
% \caption{\textbf{Training and adaptation strategies of some recent methods, as well as the datasets.} 
% }
% \label{pacsoff}
% % \vspace{-2mm}
% 	\resizebox{2\columnwidth}{!}{%
% 		\setlength\tabcolsep{4pt} 
% \begin{tabular}{lccccccc}
% \toprule
%         \multirow{2}*{Methods} & \multicolumn{2}{c}{Training distributions} & \multicolumn{2}{c}{What to adapt} \multicolumn{3}{c}{What to adaptation} \\ 
%         \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-8}
%         & Single & Multiple & Model & Sample & Iteratively update & Num of samples & Online/batch-wise \\ 
%         \midrule
%         \rowcolor{mColor2}
%         \multicolumn{8}{l}{\textbf{Fine-tuning-based model adaptation}} \\
%         \cite{sun2020test} & \ymark & ~ & \ymark & ~ & \ymark & Single/Batches & Online/sample-wise \\ 
%         \cite{wang2021tent} & \ymark & ~ & \ymark & ~ & \ymark & Batches & Online \\ 
%         \cite{zhang2021memo} & \ymark & ~  & \ymark & ~ & \ymark & Single & Sample-wise  \\ 
%         \cite{jang2022test} & \ymark & \ymark & \ymark & ~ & \ymark & Batches & Online \\ 
%         \rowcolor{mColor2}
%         \multicolumn{8}{l}{\textbf{Inferring-based model adaptation}} \\
%         \cite{dubey2021adaptive} & ~   & \ymark & \ymark & ~ & \xmark & Batches & Batch-wise \\ 
%         \cite{iwasawa2021test} & ~  & \ymark & \ymark & ~ & \xmark & Batches & Online \\ 
%         \cite{xiao2022learning} & ~  & \ymark & \ymark & ~ & \xmark & Single & Sample-wise \\
%         \rowcolor{mColor2}
%         \multicolumn{8}{l}{\textbf{Normalization-based sample adaptation}} \\
%         \cite{schneider2020improving} & \ymark & ~   & ~ & \ymark & \xmark & Batches & Batch-wise \\ 
%         \cite{du2020metanorm} & ~   & \ymark & ~ & \ymark & \xmark & Single & Sample-wise \\ 
%         \rowcolor{mColor2}
%         \multicolumn{8}{l}{\textbf{Generation-based sample adaptation}} \\
%         \cite{xiao2023energy} & ~   & \ymark & ~ & \ymark & \ymark & Single & Sample-wise \\ 
%         \cite{gao2022back} & \ymark & ~   & ~ & \ymark & \ymark & Single & Sample-wise \\ 
% \bottomrule
% \end{tabular}
% }
% \end{center}
% \end{table*}

\begin{table*}[t]
\begin{center}
\vspace{-2mm}
\caption{\textbf{Training and adaptation strategies of some recent methods, as well as the datasets.} 
}
\label{pacsoff}
% \vspace{-2mm}
	\resizebox{2\columnwidth}{!}{%
		\setlength\tabcolsep{4pt} 
\begin{tabular}{lccccccc}
\toprule
        \multirow{2}*{Methods} & \multicolumn{2}{c}{Training distributions} & \multicolumn{2}{c}{Target samples for adaptation} & \multicolumn{3}{c}{Adaptation strategy} \\ 
        \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-8} 
        & Single & Multiple & Single & Batches & Online & Batch/Sample-wise & Require iteratively update\\ 
        \midrule
        \rowcolor{mColor2}
        \multicolumn{8}{l}{\textbf{Fine-tuning-based model adaptation}} \\
        \cite{sun2020test} & \ymark & ~ & \ymark & \ymark & \ymark & \ymark & \ymark \\ 
        \cite{wang2021tent} & \ymark & ~ & ~ & \ymark & \ymark & ~ & \ymark \\ 
        \cite{zhang2021memo} & \ymark & ~  & \ymark & ~ & ~ & \ymark  & \ymark \\ 
        \cite{jang2022test} & \ymark & \ymark & ~ & \ymark & \ymark & ~ & \ymark \\ 
        \rowcolor{mColor2}
        \multicolumn{8}{l}{\textbf{Inferring-based model adaptation}} \\
        \cite{dubey2021adaptive} & ~   & \ymark & ~ & \ymark & ~ & \ymark & \xmark \\ 
        \cite{iwasawa2021test} & ~  & \ymark & ~ & \ymark & \ymark & ~ & \xmark \\ 
        \cite{xiao2022learning} & ~  & \ymark & \ymark & ~ & ~ & \ymark & \xmark \\
        \rowcolor{mColor2}
        \multicolumn{8}{l}{\textbf{Normalization-based sample adaptation}} \\
        \cite{schneider2020improving} & \ymark & ~ & ~ & \ymark & ~ & \ymark & \xmark \\ 
        \cite{du2020metanorm} & ~   & \ymark & \ymark & ~ & \ymark & ~ & \xmark \\ 
        \rowcolor{mColor2}
        \multicolumn{8}{l}{\textbf{Generation-based sample adaptation}} \\
        \cite{xiao2023energy} & ~   & \ymark & \ymark & ~ & ~ & \ymark & \ymark \\ 
        \cite{gao2022back} & \ymark & ~ & \ymark & ~ & ~ & \ymark  & \ymark \\ 
\bottomrule
\end{tabular}
}
\end{center}
\end{table*}

==> tables/adaptset.tex <==
\begin{table*}[t]
\begin{center}
\vspace{-2mm}
\caption{\textbf{Adaptation settings of some representative test-time adaptation methods.} 
}
\label{adaptset}
% \vspace{-2mm}
	\resizebox{2\columnwidth}{!}{%
		\setlength\tabcolsep{4pt} 
\begin{tabular}{lcccccc}
\toprule
        \multirow{2}*{Methods} & \multicolumn{2}{c}{Inference strategy} & \multicolumn{4}{c}{Inference data} \\
        \cmidrule(lr){2-3} \cmidrule(lr){4-7}
        & Iterative & On-the-fly & Online & Batch-wise & Sample-wise & Dynamic \\ 
        \midrule
        \multirow{3}*{Model adaptation} & \cite{sun2020test, liu2021ttt++, gandelsmantest2022test, li2021test, osowiechi2023tttflow, cohen2020self}, & \multirow{3}*{-} & \cite{sun2020test, wang2021tent, jang2022test} & \multirow{3}*{-} & \cite{sun2020test, zhang2021memo} & \cite{wang2022continual, yuan2023robust, dobler2023robust}\\ 
        & \cite{wang2021tent, song2023ecotta, tang2023neuro, lee2022surgical, chen2023improved}, & & \cite{liu2021ttt++, zhou2021bayesian, goyal2022test} & & \cite{sain2022sketch3t, min2023meta} & \cite{brahma2022probabilistic, chakrabarty2023sata, hong2023mecta} \\
        & \cite{wang2022continual, jang2022test, boudiaf2022parameter, wang2023feature, su2022revisiting} & & \cite{chen2022contrastive, lee2022surgical} & & \cite{alet2021tailoring, bartler2022mt3, lin2022video} & \cite{niu2022efficient, niu2023towards, song2023ecotta} \\
        \midrule
        Inference adaptation  & - & \cite{iwasawa2021test, zhang2023adanpc, dubey2021adaptive, xiao2022learning, yeo2023rapid} & \cite{iwasawa2021test, huangextrapolative, zhang2023adanpc} & \cite{dubey2021adaptive, yeo2023rapid} & \cite{xiao2022learning, wang2023dynamically, sun2022dynamic} & - \\ \midrule
        \multirow{3}*{Normalization adaptation}  & \multirow{3}*{-} & \cite{gong2022note, nado2020evaluating} & \cite{yang2022test, mirza2022norm} & \cite{schneider2020improving, zhang2021adaptive} & \cite{du2020metanorm, jiang2023domain} & \multirow{3}*{-} \\
        & & \cite{schneider2020improving, lim2023ttn} & \cite{hong2023mecta, zhao2023delta} & \cite{nado2020evaluating, lim2023ttn} & \cite{khurana2021sita, mirza2022norm, hu2021mixnorm} & \\
        & & \cite{du2020metanorm} & & \cite{you2021test} & \cite{kaku2020like, gong2022note} & \\ \midrule
        Sample adaptation  & \cite{gao2022back, xiao2023energy, pandey2021generalization, huang2020neural, yuan2024tea} & \cite{park2023test} & - & - & \cite{gao2022back, xiao2023energy, pandey2021generalization, huang2020neural, yuan2024tea, park2023test} & - \\ \midrule
        \multirow{2}*{Prompt adaptation}  & \cite{shu2022test, ma2024swapprompt, yoon2024c, gao2022visual, sun2023vpa, samadh2023align} & \multirow{2}*{\cite{fahes2023poda, roth2023waffling, ren2024chatgpt, mirza2024meta, xiao2024any}} & \multirow{2}*{-} & \multirow{2}*{-} & \cite{shu2022test, ma2024swapprompt} & \multirow{2}*{-}\\
        & \cite{zhang2022tempera, manas2024improving, fahes2023poda, zhao2024test} & & & & \cite{samadh2023align, yoon2024c} & \\
\bottomrule
\end{tabular}
}
\end{center}
\end{table*}

==> tables/testtable.tex <==
\begin{table}[htbp]
    \centering
    \begin{tabular}{ccccc}
    \hline
    A & B & C & D & E \\
    \hline
    1 & 2 & 3 & 4 & 5 \\
    \hline
    6 & \multicolumn{3}{c}{
        \multirow{3}{*}{
            \parbox[c][2.5cm][c]{6cm}{ % Underlying text
                \centering
                % Original Text Spanning 3x3 Area
                \begin{tikzpicture}[overlay,remember picture]
                    \node[fill=gray!40,opacity=0.5,rounded corners=2pt,text opacity=1,minimum width=6cm,minimum height=1cm,anchor=center] at (0,0.8) {future opportunity};
                \end{tikzpicture}
            }
        }
    } & 10 \\ \hline
    \cline{1-1} \cline{5-5}
    7 &  &  &  & 11 \\
    \cline{1-1} \cline{5-5}
    8 &  &  &  & 12 \\
    \hline
    9 & 13 & 14 & 15 & 16 \\
    \hline
    \end{tabular}
    \caption{Table with Future Opportunity Text over Original Content}
\end{table}


==> tables/trainingset.tex <==
\begin{table*}[t!]
\begin{center}
\vspace{-2mm}
\caption{\textbf{Training settings of some representative test-time adaptation methods.} 
\cs{Table is still a bit boring, need to think a bit about it.}}
\label{trainingset}
% \vspace{-2mm}
	\resizebox{2\columnwidth}{!}{%
		\setlength\tabcolsep{4pt} 
\begin{tabular}{llccc}
\toprule
        Methods & Preparation-agnostic & Training preparation & Training \& Data preparation \\ 
        \midrule
        \multirow{3}*{Model adaptation} & \cite{wang2021tent, zhou2021bayesian, tang2023neuro, fleuret2021test, zhang2021memo, niu2022efficient, niu2023towards},
        &
        \multirow{3}*{\cite{liu2021ttt++, gandelsmantest2022test, li2021test, osowiechi2023tttflow, cohen2020self, sun2020test}} & \multirow{3}*{\cite{alet2021tailoring, bartler2022mt3, chi2021test, cho2023complementary, choi2021test, hatem2023point, liu2023meta, min2023meta, zhong2022meta}} \\ 
        & \cite{wang2023feature, su2022revisiting, su2023revisiting, jung2022cafa, fleuret2021test, fang2013video}, & & \\
        & \cite{rusak2021if, wang2022continual, chen2022contrastive, jang2022test, boudiaf2022parameter}, & & \\
        \midrule
        Inference adaptation & \cite{iwasawa2021test, huangextrapolative, zhang2023adanpc} &
        \cite{dubey2021adaptive, kim2022variational, yeo2023rapid, wang2023dynamically} & \cite{xiao2022learning, sun2022dynamic} \\ 
        \midrule
        Normalization adaptation & \cite{gong2022note, kaku2020like, li2016revisiting, nado2020evaluating}
        \cite{schneider2020improving, khurana2021sita, you2021test, hu2021mixnorm, yang2022test} & \cite{lim2023ttn}  &  \cite{du2020metanorm, zhang2021adaptive, xu2022mimic}  \\
        \midrule
        Sample adaptation & - &
        \cite{gao2022back, pandey2021generalization, nie2022diffusion, huang2020neural, yuan2024tea}   & \cite{xiao2023energy, park2023test} \\ 
        \midrule
        Prompt adaptation & \cite{shu2022test, yoon2024c, gao2022visual, sun2023vpa, fahes2023poda, zhang2022tempera, ma2024swapprompt, samadh2023align, zhao2024test} & - & \cite{xiao2024any} \\ 
\bottomrule
\end{tabular}
}
\end{center}
\end{table*}
